SemCal: Semantic LiDAR-Camera Calibration using Neural MutualInformation Estimator

This paper proposes SemCal: an automatic, targetless, extrinsic calibration algorithm for a LiDAR and camera system using semantic information. We leverage a neural information estimator to estimate the mutual information (MI) of semantic information extracted from each sensor measurement, facilitating semantic-level data association. By using a matrix exponential formulation of the $se(3)$ transformation and a kernel-based sampling method to sample from camera measurement based on LiDAR projected points, we can formulate the LiDAR-Camera calibration problem as a novel differentiable objective function that supports gradient-based optimization methods. We also introduce a semantic-based initial calibration method using 2D MI-based image registration and Perspective-n-Point (PnP) solver. To evaluate performance, we demonstrate the robustness of our method and quantitatively analyze the accuracy using a synthetic dataset. We also evaluate our algorithm qualitatively on an urban dataset (KITTI360) and an off-road dataset (RELLIS-3D) benchmark datasets using both hand-annotated ground truth labels as well as labels predicted by the state-of-the-art deep learning models, showing improvement over recent comparable calibration approaches.

==> equations/H.tex <==
\begin{equation}
    H = \sum_{i=0}^{5} {v_iB_i}
\label{eq:h}
\end{equation}

==> equations/T.tex <==
\begin{equation}
T =  \exp{(\sum_{i=0}^{5} {v_iB_i})} = \sum_{j=0}^{\infty } { \frac{(\sum_{i=0}^{5} {v_iB_i})^n }{n!} }
\end{equation}

==> equations/cyproj.tex <==
\begin{equation}
\label{eq:cyproj}
    \begin{pmatrix}
      u \\ v
    \end{pmatrix}=
    \begin{pmatrix}
      \frac{1}{2}[1-arctan(y,x)\pi ^{-1}]w \\
      [1-(arcsin(zr^{-1})+f_{up})f^{-1}]h
    \end{pmatrix}
\end{equation}

==> equations/generators.tex <==
\begin{equation}
\begin{matrix}
B_0 = \begin{pmatrix}
0 & 0 & 0 & 1 \\ 
0 & 0 & 0 & 0 \\ 
0 & 0 & 0 & 0 \\ 
0 & 0 & 0 & 0
\end{pmatrix} & 
B_1 = \begin{pmatrix}
0 & 0 & 0 & 0 \\ 
0 & 0 & 0 & 1 \\ 
0 & 0 & 0 & 0 \\ 
0 & 0 & 0 & 0
\end{pmatrix}\\ 
 & \\ 
B_2 = \begin{pmatrix}
0 & 0 & 0 & 0 \\ 
0 & 0 & 0 & 0 \\ 
0 & 0 & 0 & 1 \\ 
0 & 0 & 0 & 0
\end{pmatrix} & 
B_3 = \begin{pmatrix}
0 & 0 & 0 & 0 \\ 
0 & 0 & -1 & 0 \\ 
0 & 1 & 0 & 0 \\ 
0 & 0 & 0 & 0
\end{pmatrix}\\ 
 & \\ 
B_4 = \begin{pmatrix}
0 & 0 & 0 & 1 \\ 
0 & 0 & 0 & 0 \\ 
0 & 0 & 0 & 0 \\ 
-1 & 0 & 0 & 0
\end{pmatrix} & 
B_5 = \begin{pmatrix}
0 & -1 & 0 & 0 \\ 
1 & 0 & 0 & 0 \\ 
0 & 0 & 0 & 0 \\ 
0 & 0 & 0 & 0
\end{pmatrix}
\end{matrix}
\label{eq:se3_basis}
\end{equation}

==> equations/lidar2cam.tex <==
\begin{equation}
z^C_i  \begin{bmatrix}p^{uv}_{i}\\1\\0\end{bmatrix} = \begin{bmatrix}p_i^C\\0\end{bmatrix}  = \begin{bmatrix}K&0\\0&1\end{bmatrix} \begin{bmatrix}R&t\\0&0\end{bmatrix}\begin{bmatrix}p^L_i\\1\end{bmatrix} 
\label{eq:lidarcam}
\end{equation}

\begin{itemize}
    \item $p_i^L=\begin{bmatrix}x_{i}^L&y_{i}^L&z_{i}^L\end{bmatrix}^T$ represents the coordinate of point $p_i$ in Lidar local frame;
    %\item $t = \begin{bmatrix}t_{x}&y_{y}&t_{z}\end{bmatrix}^T$ represents translation vector;
    \item $t$ represents the $3\times1$ translation vector;
    \item $R$ represents the $3\times3$ rotation matrix;
    %\item $R =  \begin{bmatrix}r_{11}&r_{12}&r_{13}\\r_{21}&r_{22}&r_{23}\\r_{31}&r_{32}&r_{33}\end{bmatrix} $ represents rotation matrix;  
    %\item $K =   \begin{bmatrix}f_{x}&0&c_{x}\\0&f_{y}&c_{y}\\0&0&1\end{bmatrix}  $ represents intrinsic calibration matrix of camera;  
    \item $K$ represents the $3\times3$ intrinsic matrix of camera;
    \item $p_i^C=\begin{bmatrix}x_{i}^C&y_{i}^C&z_{i}^C\end{bmatrix}^T$ represents the coordinate of point $p_i$ in Camera local frame;
    \item $p_i^{uv}=\begin{bmatrix}u_{i}&v_{i}\end{bmatrix}^T$ represents the coordinate of point $p_i$ in the camera projection plane;
\end{itemize}

==> equations/mi.tex <==
\begin{equation}
I(X;Z) := H(X)-H(X|Z)
\end{equation}

==> equations/mi_est.tex <==
\begin{equation}
I(X,Y) = MI(\widetilde{L}^{C},\widetilde{L}^{L})
\label{eq:mi_est}
\end{equation}

==> equations/proj.tex <==
\begin{equation}
P^{uv} = Proj(P^{L},R,t)
\label{eq:proj}
\end{equation}

==> figures/kitti360.tex <==
\begin{figure}[]
  \centering
    \begin{tabular}{cc}
    \centering
     (a) &   \includegraphics[width=0.4\textwidth]{images/kitti360/gt.png} \\
     (b) &  \includegraphics[width=0.4\textwidth]{images/kitti360/soic.png}\\
     (c) &  \includegraphics[width=0.4\textwidth]{images/kitti360/gray.png}\\
     (d) &  \includegraphics[width=0.4\textwidth]{images/kitti360/mime.png}\\
    \end{tabular}
    \caption{Calibration Results on KITTI360 dataset (a) Ground Truth, (b) SOIC, (c) Gray Scale, (d) Semantic }    
    \label{fig:kitti360}
\end{figure}


==> figures/rellis3d.tex <==
\begin{center}
\begin{figure}[]
  \centering
    \begin{tabular}{cc}
    %\centering
     \centering (a) &   \includegraphics[width=0.4\textwidth]{images/rellis3d/gt.png} \\
     (b) &  \includegraphics[width=0.4\textwidth]{images/rellis3d/soic.png}\\
     (c) &  \includegraphics[width=0.4\textwidth]{images/rellis3d/gray.png}\\
     (d) &  \includegraphics[width=0.4\textwidth]{images/rellis3d/mime.png}\\
    \end{tabular}
    \caption{Hill Example (a) RGB Image, (b) Image Label, (c) Single Scan, (d) Multiple Scans}    
    \label{fig:rellis3d}
\end{figure}

\end{center}


==> sections/05_discussion.tex <==
\section{Discussion}

